Online Authentication Habits of Indian Users

Passwords have been long used as the primary authentication method for web services. Weak passwords used by the users have prompted the use of password management tools and two-factor authentication to ensure better account security. While prior studies have studied their adoption individually, none of these studies focuses particularly on the Indian setting, which is culturally and economically different from the countries in which these studies have been done in the past. To this end, we conducted a survey with 90 participants residing in India to better understand the mindset of people on using password managers and two-factor authentication (2FA). Our findings suggest that a majority of the participants have used 2FA and password managers in some form, although they are sometimes unaware of their formal names. While many participants used some form of 2FA across all their accounts, browser-integrated and device-default password managers are predominantly utilized for less sensitive platforms such as e-commerce and social media rather than for more critical accounts like banking. The primary motivation for using password managers is the convenience of auto-filling. However, some participants avoid using password managers due to a lack of trust in these tools. Notably, dedicated third-party applications show low adoption for both password manager and 2FA. Despite acknowledging the importance of secure password practices, many participants still reuse passwords across multiple accounts, prefer shorter passwords, and use commonly predictable password patterns. Overall, the study suggests that Indians are more inclined to choose default settings, underscoring the need for tailored strategies to improve user awareness and strengthen password security practices.

==> results-extra.tex <==


\begin{figure}[H]
    \centering
    \begin{minipage}{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/accounts-of-participants.png}
        \caption{Distribution of Online Accounts Owned by Participants}
        \label{fig:graph-number-accounts}
    \end{minipage}
        \begin{minipage}{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/device-used-count.png}
        \caption{Distribution of Primary Devices Used by Participants to Access the Web (Multiple Selections Allowed)}
        \label{fig:graph-number-accounts}
    \end{minipage}
\end{figure}

\begin{figure}[H]
    \centering
    \begin{minipage}{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/accounts-created-by-others.png}
        \caption{Distribution of Online Accounts Created by Others for the Participants}
        \label{fig:graph-account-created-by-others}
    \end{minipage}
        \begin{minipage}{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/frequency-login-pass.png}
        \caption{Daily Variation in Unique Passwords}
        \label{fig:graph-freq-login-pass}
    \end{minipage}
\end{figure}

\begin{figure}[H]
    \centering
    \begin{minipage}{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/number-diff-pass-daily.png}
        \caption{Count of Different Passwords Used by the Participants Daily}
        \label{fig:graph-diff-pass-daily}
    \end{minipage}
        \begin{minipage}{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/number-diff-pass-monthly.png}
        \caption{Monthly Variation in Unique Passwords}
        \label{fig:graph-diff-pass-monthly}
    \end{minipage}
    
\end{figure}

\begin{figure}[H]
    \centering
    \begin{minipage}{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/forgotten-password.png}
        \caption{Password Forgetfulness: Participant Statistics}
        \label{fig:graph-forgot-pass}
    \end{minipage}
\end{figure}
\begin{figure}[H]
    \centering
    \begin{minipage}{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/pass-stored-elec.png}
        \caption{Passwords Noted Electronically by the Participants}
        \label{fig:graph-pass-stored-elec}
    \end{minipage}
        \begin{minipage}{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/pass-stored-phys.png}
        \caption{Passwords Stored Physically by the Participants}
        \label{fig:graph-stored-pass-phys}
    \end{minipage}
\end{figure}

\begin{figure}[H]
    \centering
    \begin{minipage}{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/freq-pass-change.png}
        \caption{Frequency of Password Changing among Participants}
        \label{fig:graph-freq-pass-change}
    \end{minipage}
        \begin{minipage}{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/pass-template.png}
        \caption{Participants having Password Templates for Creating their New Passwords}
        \label{fig:graph-pass-template}
    \end{minipage}
\end{figure}
